ProfilingAgent: Profiling-Guided Agentic Reasoning for Adaptive Model Optimization

Foundation models face growing compute and memory bottlenecks, hindering deployment on resource-limited platforms. While compression techniques such as pruning and quantization are widely used, most rely on uniform heuristics that ignore architectural and runtime heterogeneity. Profiling tools expose per-layer latency, memory, and compute cost, yet are rarely integrated into automated pipelines. We propose ProfilingAgent, a profiling-guided, agentic approach that uses large language models (LLMs) to automate compression via structured pruning and post-training dynamic quantization. Our modular multi-agent system reasons over static metrics (MACs, parameter counts) and dynamic signals (latency, memory) to design architecture-specific strategies. Unlike heuristic baselines, ProfilingAgent tailors layer-wise decisions to bottlenecks. Experiments on ImageNet-1K, CIFAR-10, and CIFAR-100 with ResNet-101, ViT-B/16, Swin-B, and DeiT-B/16 show pruning maintains competitive or improved accuracy (about 1% drop on ImageNet-1K, +2% gains for ViT-B/16 on smaller datasets), while quantization achieves up to 74% memory savings with <0.5% accuracy loss. Our quantization also yields consistent inference speedups of up to 1.74 times faster. Comparative studies with GPT-4o and GPT-4-Turbo highlight the importance of LLM reasoning quality for iterative pruning. These results establish agentic systems as scalable solutions for profiling-guided model optimization.

==> name.tex <==
% Example bibliography entries (add these to your .bib file)
% \begin{thebibliography}{1}
% \bibitem{profiling_bottleneck} S. S. S. S. et al., "Profiling and Bottleneck Identification for Large Language Model Fine-Tuning," Supercomputing 2024 Poster.
% \bibitem{study_optimizations} S. S. S. S. et al., "A Study of Optimizations for Fine-tuning Large Language Models," arXiv preprint arXiv:2406.02290, 2024.
% \bibitem{moe_guide} M. Grootendorst, "A Visual Guide to Mixture of Experts (MoE)," 2024.
% \bibitem{gpu_bottlenecks} P. G. Recasens et al., "Mind the Memory Gap: Unveiling GPU Bottlenecks in Large-Batch LLM Inference," arXiv preprint arXiv:2503.08311, 2025.
% \bibitem{adaline_attention} Adaline.ai, "Understanding Attention Mechanisms in LLMs," 2025.
% \bibitem{fastgen_msft} Microsoft Research, "LLM Profiling Guides KV Cache Optimization (FastGen)," 2024.
% \bibitem{fastgen_marktechpost} Marktechpost, "FastGen: Cutting GPU Memory Costs Without Compromising on LLM Quality," 2024.
% \end{thebibliography}


% S. S. S. S. et al., "Profiling and Bottleneck Identification for Large Language Model Fine-Tuning," Supercomputing 2024 Poster. [Online]. Available: https://sc24.supercomputing.org/proceedings/posters/poster_files/spost154s2-file2.pdf

% S. S. S. S. et al., "A Study of Optimizations for Fine-tuning Large Language Models," arXiv preprint arXiv:2406.02290, 2024. [Online]. Available: https://arxiv.org/abs/2406.02290

% M. Grootendorst, "A Visual Guide to Mixture of Experts (MoE)," 2024. [Online]. Available: https://www.maartengrootendorst.com/blog/mixture-of-experts/

% P. G. Recasens, S. S. S. S., and S. S. S. S., "Mind the Memory Gap: Unveiling GPU Bottlenecks in Large-Batch LLM Inference," arXiv preprint arXiv:2503.08311, 2025. [Online]. Available: https://arxiv.org/abs/2503.08311

% Adaline.ai, "Understanding Attention Mechanisms in LLMs," 2025. [Online]. Available: https://adaline.ai/understanding-attention-mechanisms-in-llms/

% Microsoft Research, "LLM Profiling Guides KV Cache Optimization (FastGen)," 2024. [Online]. Available: https://www.microsoft.com/en-us/research/blog/llm-profiling-guides-kv-cache-optimization/

% Marktechpost, "FastGen: Cutting GPU Memory Costs Without Compromising on LLM Quality," 2024. [Online]. Available: https://www.marktechpost.com/2024/03/21/fastgen-cutting-gpu-memory-costs-without-compromising-on-llm-quality/


==> url.tex <==
https://www.microsoft.com/en-us/research/blog/llm-profiling-guides-kv-cache-optimization/

https://arxiv.org/pdf/2503.08311


https://arxiv.org/pdf/2410.19456v1


https://openreview.net/pdf?id=RC5FPYVQaH

https://www.cudocompute.com/blog/what-is-the-cost-of-training-large-language-models

https://arxiv.org/pdf/2503.12434v1

https://research.ibm.com/publications/profile-based-detection-of-layered-bottlenecks


https://sc24.supercomputing.org/proceedings/poster/poster_files/post269s2-file3.pdf



https://arxiv.org/pdf/2408.04693v1
